Vortex: Extending the RISC-V ISA for GPGPU and 3D-GraphicsResearch

The importance of open-source hardware and software has been increasing. However, despite GPUs being one of the more popular accelerators across various applications, there is very little open-source GPU infrastructure in the public domain. We argue that one of the reasons for the lack of open-source infrastructure for GPUs is rooted in the complexity of their ISA and software stacks.In this work, we first propose an ISA extension to RISC-V that supports GPGPUs and graphics. The main goal of the ISA extension proposal is to minimize the ISA changes so that the corresponding changes to the open-source ecosystem are also minimal, which makes for a sustainable development ecosystem. To demonstrate the feasibility of the minimally extended RISC-V ISA, we implemented the complete software and hardware stacks of Vortex on FPGA. Vortex is a PCIe-based soft GPU that supports OpenCL and OpenGL.Vortex can be used in a variety of applications, including machine learning, graph analytics, and graphics rendering. Vortex can scale up to 32 cores on an Altera Stratix 10 FPGA, delivering a peak performance of 25.6 GFlops at 200 Mhz.

==> 999.TODO.tex <==
Adding more info for the paper

Extensions of CSR 
- extending CSR to include thread id information. 
-Number of cores, number or warps 




==============
More experiments 
- Different W-T trade-off. 
Current version, 8W-2T shows the best performance/area 
more higher number of threads? 
the trade-off needs to include different number of cores 

- More benchmarks 

- Having many single core and measure parallelized version (1W-1T case) 

- Graphics benchmark suite 

====
More explanations 
Driver section 
Compiler section 

Graphics pipeline sw interface vs. hardware 


==> key_points.tex <==
- first draft should focus on citation references and comparison data

- dataflow-based accelerators ubiquitous FPGAs.

- prioritizing scalability of cores versus features for IPC.
- elastic skid buffer types
- history of soft-gpu and comparison with Vortex
- 

Background
 1- GPU ISA improvements accross al vendors
 2- Accelerators on FPGAs
 3-

Elastic pipelines
 - components reuse
 - skid buffer types
 - scalability of the system to 32 cores
 - tracing and debugging of components/system leveraging valid/ready standard protocol

Evaluation:
- Determining the optimal architecture: Warp=4, threads=4, 

References:
FlexGrip - A Soft GPGPU for FPGAs
NyuziRaster - Optimizing Rasterizer Performance and Energy in the Nyuzi Open Source GPU
Automatic Generation of Efficient Accelerators for Reconfigurable Hardware


==> roadmap.tex <==
\section{Roadmap}



==> scratchpad.tex <==
\section{Scatchpad}
